Two-level trust-region method with random subspaces

We introduce a two-level trust-region method (TLTR) for solving unconstrained nonlinear optimization problems. Our method uses a composite iteration step, which is based on two distinct search directions. The first search direction is obtained through minimization in the full/high-resolution space, ensuring global convergence to a critical point. The second search direction is obtained through minimization in the randomly generated subspace, which, in turn, allows for convergence acceleration. The efficiency of the proposed TLTR method is demonstrated through numerical experiments in the field of machine learning

==> references.tex <==
\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{Conn TRmethods} Conn, A. R. ; Gould, N. I. M. and Toint, P. L.: Trust Region Methods.
Society for Industrial and Applied Mathematics, doi: 10.1137/1.9780898719857 (2000).


% @book{doi:10.1137/1.9780898719857,
% author = {Conn, Andrew R. and Gould, Nicholas I. M. and Toint, Philippe L.},
% title = {Trust Region Methods},
% publisher = {Society for Industrial and Applied Mathematics},
% year = {2000},
% doi = {10.1137/1.9780898719857},
% address = {},
% edition   = {},
% URL = {https://epubs.siam.org/doi/abs/10.1137/1.9780898719857},
% eprint = {https://epubs.siam.org/doi/pdf/10.1137/1.9780898719857}
% }

\bibitem{Conn MTR} Conn, A. R. ; Vicente, L. N. and Visweswariah, C., A. R.; Gould, N. I. M. and Toint, P. L.: Two-Step Algorithms for Nonlinear Optimization with Structured Applications.
SIAM Journal on Optimization, vol 9,doi:10.1137/S1052623498334396(1999).
% @article{doi:10.1137/S1052623498334396,
% author = {Conn, Andrew R. and Vicente, Lu\'{\i}s N. and Visweswariah, Chandu},
% title = {Two-Step Algorithms for Nonlinear Optimization with Structured Applications},
% journal = {SIAM Journal on Optimization},
% volume = {9},
% number = {4},
% pages = {924-947},
% year = {1999},
% doi = {10.1137/S1052623498334396},

% URL = { https://doi.org/10.1137/S1052623498334396
% },
% eprint = { https://doi.org/10.1137/S1052623498334396
% }

% @Book{NoceWrig06,
%   author    = {Jorge Nocedal and Stephen J. Wright},
%   publisher = {Springer},
%   title     = {Numerical Optimization},
%   year      = {2006},
%   address   = {New York, NY, USA},
%   edition   = {2e},
% }
\bibitem{trottenberg2000multigrid} Trottenberg, U. and Oosterlee, C. W. and Schuller, A. : Multigrid.
Elsevier, (2000).

% @book{trottenberg2000multigrid,
%   title={Multigrid},
%   author={Trottenberg, Ulrich and Oosterlee, Cornelius W and Schuller, Anton},
%   year={2000},
%   publisher={Elsevier}
% }
\bibitem{Nocedal} Nocedal, J. and Wright S. J. : Numerical Optimization.
Springer, doi: https://doi.org/10.1007/978-0-387-40065-5 (2006).


\bibitem{Fletcher1982} Fletcher, R.: Second order corrections for non-differentiable optimization.
Numerical Analysis,
pp. 85-114.  Pringer Berlin Heidelberg doi: 10.1007/BFb0093151 (1982).

% @InProceedings{10.1007/BFb0093151,
% author="Fletcher, R.",
% editor="Watson, G. Alistair",
% title="Second order corrections for non-differentiable optimization",
% booktitle="Numerical Analysis",
% year="1982",
% publisher="Springer Berlin Heidelberg",
% address="Berlin, Heidelberg",
% pages="85--114",
% isbn="978-3-540-39009-1"
% }

\bibitem{More} Mor\'{e}, J. J. and and Sorensen, D. C. : Computing a Trust Region Step.
SIAM Journal on Scientific and Statistical Computing, vol. 4 pp. 553-572. doi: 10.1137/0904038 (1983).

% @article{doi:10.1137/0904038,
% author = {Mor\'{e}, Jorge J. and Sorensen, D. C.},
% title = {Computing a Trust Region Step},
% journal = {SIAM Journal on Scientific and Statistical Computing},
% volume = {4},
% number = {3},
% pages = {553-572},
% year = {1983},
% doi = {10.1137/0904038},

% URL = { 
%         https://doi.org/10.1137/0904038
% },
\bibitem{Yuan1985} Yuan, Y.: On the superlinear convergence of a trust region algorithm for nonsmooth optimization.
Mathematical Programming,  vol 31,
pp. 269-285. Springer, Verlag (1985).
% @article{yuan1985superlinear,
%   title={On the superlinear convergence of a trust region algorithm for nonsmooth optimization},
%   author={Yuan, Y-X},
%   journal={Mathematical Programming},
%   volume={31},
%   pages={269--285},
%   year={1985},
%   publisher={Springer-Verlag}
% }
\bibitem{TRsubproblems} Gould, N. I. M. and Lucidi, S. and Roma, M. and Toint, P. L.: Solving the Trust-Region Subproblem using the Lanczos Method.
SIAM Journal on Optimization,  vol 9,
pp. 504-525. doi: 10.1137/S1052623497322735 (1999).

% @article{doi:10.1137/S1052623497322735,
% author = {Gould, Nicholas I. M. and Lucidi, Stefano and Roma, Massimo and Toint, Philippe L.},
% title = {Solving the Trust-Region Subproblem using the Lanczos Method},
% journal = {SIAM Journal on Optimization},
% volume = {9},
% number = {2},
% pages = {504-525},
% year = {1999},
% doi = {10.1137/S1052623497322735},

% URL = { 
    
%         https://doi.org/10.1137/S1052623497322735
    
% },
% }

\bibitem{Cartis} Cartis, C. and Fiala, J. and Shao, Z.: Randomised subspace methods for non-convex optimization, with applications to nonlinear least-squares.
arXiv e-prints (2022).
% @misc{cartis2022randomised,
%   title={Randomised subspace methods for non-convex optimization, with applications to nonlinear least-squares. arXiv e-prints},
%   author={Cartis, C and Fiala, J and Shao, Z},
%   year={2022},
%   publisher={preparation}
% }


\bibitem{Nesterov} Nesterov, Y.: Efficiency of Coordinate Descent Methods on Huge-Scale Optimization Problems.
SIAM Journal on Optimization,  vol 22,
pp. 341-362. doi: 10.1137/100802001(2012).

% @article{doi:10.1137/100802001,
% author = {Nesterov, Yu.},
% title = {Efficiency of Coordinate Descent Methods on Huge-Scale Optimization Problems},
% journal = {SIAM Journal on Optimization},
% volume = {22},
% number = {2},
% pages = {341-362},
% year = {2012},
% doi = {10.1137/100802001},
% URL = { 
%         https://doi.org/10.1137/100802001

% },
% eprint = { 
%         https://doi.org/10.1137/100802001
% }

\bibitem{Lindenstrauss} Johnson, W.B. and Lindenstrauss and J. and Schechtman, G.: Extensions of lipschitz maps into Banach spaces. Israel J. Math. 
vol. 54, 129–138  doi:10.1007/BF02764938 (1986).

% TY  - JOUR
% AU  - Johnson, William B.
% AU  - Lindenstrauss, Joram
% AU  - Schechtman, Gideon
% PY  - 1986
% DA  - 1986/06/01
% TI  - Extensions of lipschitz maps into Banach spaces
% JO  - Israel Journal of Mathematics
% SP  - 129
% EP  - 138
% VL  - 54
% IS  - 2
% AB  - It is proved that ifY ⊂X are metric spaces withY havingn≧2 points then any mapf fromY into a Banach spaceZ can be extended to a map$$\hat f$$fromX intoZ so that$$\left\| {\hat f} \right\|_{lip}  \leqq c log n\left\| f \right\|_{lip} $$wherec is an absolute constant. A related result is obtained for the case whereX is assumed to be a finite-dimensional normed space andY is an arbitrary subset ofX.
% SN  - 1565-8511
% UR  - https://doi.org/10.1007/BF02764938
% DO  - 10.1007/BF02764938
% ID  - Johnson1986
% ER  - 

\bibitem{sketchingGD} Kozak, D. and Becker, S. and Doostan, A. and Tenorio, L.: A stochastic subspace approach to gradient-free optimization in high dimensions. 
Computational Optimization and Applications vol. 79, 339–368  doi:10.1007/s10589-021-00271-w (2021).

% TY  - JOUR
% AU  - Kozak, David
% AU  - Becker, Stephen
% AU  - Doostan, Alireza
% AU  - Tenorio, Luis
% PY  - 2021
% DA  - 2021/06/01
% TI  - A stochastic subspace approach to gradient-free optimization in high dimensions
% JO  - Computational Optimization and Applications
% SP  - 339
% EP  - 368
% VL  - 79
% IS  - 2
% SN  - 1573-2894
% UR  - https://doi.org/10.1007/s10589-021-00271-w
% DO  - 10.1007/s10589-021-00271-w
% ID  - Kozak2021

\bibitem{newtonSketch} Pilanci, M. and Wainwright, M. : Newton Sketch: A Near Linear-Time Optimization Algorithm with Linear-Quadratic Convergence.
SIAM Journal on Optimization vol. 27, 205-245 doi:10.1137/15M1021106 (2017).

% @article{doi:10.1137/15M1021106,
% author = {Pilanci, Mert and Wainwright, Martin J.},
% title = {Newton Sketch: A Near Linear-Time Optimization Algorithm with Linear-Quadratic Convergence},
% journal = {SIAM Journal on Optimization},
% volume = {27},
% number = {1},
% pages = {205-245},
% year = {2017},
% doi = {10.1137/15M1021106},
% URL = { 
%         https://doi.org/10.1137/15M1021106
% },
% eprint = {
%         https://doi.org/10.1137/15M1021106
% }
\bibitem{Griewank1982} Griewank, A. and Toint, Ph. L.: Partitioned variable metric updates for large structured optimization problems. Numerische Mathematik, vol 39, pp. 119-137, doi:10.1007/BF01399316 (1982).



\end{thebibliography}
